Pano360: Perspective to Panoramic Vision with Geometric Consistency

Prior panorama stitching approaches heavily rely on pairwise feature correspondences and are unable to leverage geometric consistency across multiple views. This leads to severe distortion and misalignment, especially in challenging scenes with weak textures, large parallax, and repetitive patterns. Given that multi-view geometric correspondences can be directly constructed in 3D space, making them more accurate and globally consistent, we extend the 2D alignment task to the 3D photogrammetric space. We adopt a novel transformer-based architecture to achieve 3D awareness and aggregate global information across all views. It directly utilizes camera poses to guide image warping for global alignment in 3D space and employs a multi-feature joint optimization strategy to compute the seams. Additionally, to establish an evaluation benchmark and train our network, we constructed a large-scale dataset of real-world scenes. Extensive experiments show that our method significantly outperforms existing alternatives in alignment accuracy and perceptual quality.

==> tables/camera.tex <==
{
  \centering
  \makeatletter
  % 1. 设置编号前缀为 A，并手动设定序号为 1
  \renewcommand{\thetable}{A\arabic{table}}
  \setcounter{table}{0}
  \def\@captype{table}
  \makeatother
  \footnotesize
  \setlength{\tabcolsep}{6pt}
  \renewcommand{\arraystretch}{0.9} % 稍微增加行间距，视觉更舒适
  
  % 2. 插入你要求的中文描述作为标题 (注意 & 符号需要加反斜杠 \&)
  \captionof{table}{\textbf{Comparison of pose accuracy on Pano360.}} 
\label{tab:camera}
  \begin{tabular}{ccccc}
    \toprule
    Methods & AUC@15$\uparrow$ & BRIS$\downarrow$ & NIQE$\downarrow$ & Time \\
    \midrule
    COLMAP (SIFT+NN) & 65.4 & 43.8 & 4.51 & $>$ 20s \\
    COLMAP (SPSG)    & 77.6 & 38.7 & 3.70 & $>$ 30s \\
    Ours (Feed-Forward) & 87.2 & 32.1 & 3.42 & $\sim$ \textbf{5.2}s \\
    Ours (with BA)   & \textbf{93.7} & \textbf{31.1} & \textbf{3.28} & $\sim$ 9.6s \\
    \bottomrule
  \end{tabular}
}

==> tables/memory.tex <==
% {
%     \centering
%     \footnotesize 
%     \setlength{\tabcolsep}{6pt}       % 控制列宽
%     \renewcommand{\arraystretch}{1.0} % 行间距设为1.0（紧凑默认值）

%     \begin{tabular}{ccccccccc}
%       \toprule
%       % === 表头 ===
%       % 1. 直接写数字
%       % 2. \\[-0.5ex] 意思是：换行后，向上回缩 0.5个字符高度，让 \midrule 贴得更近
%       % Input Frames & 2 & 4 & 8 & 10 & 20 & 24 & 48 & 64\\[-0.3ex]
      
%       % \midrule
      
%       % % === 数据 ===
%       % Time (s)    & 0.7 & 4.1 & 12.7 & 16.4 & 28.7 & 34.5 & 55.0 & 73.0\\
%       % Mem. (GB)    & 7.62 & 8.58 & 10.8 & 11.3 & 13.9 & 14.9 & 26.4 & 42.2\\
%       % SSIM (\%)    & 95.5 & 95.1 & 94.6 & 94.5 & 93.2 & 93.8 & $-$  & $-$  \\ 
%       Input Frames & 2 & 4 & 8 & 10 & 16 & 20 & 24 \\[-0.3ex]
      
%       \midrule
      
%       % === 数据 ===
%       Time (s)    & 0.7 & 2.7 & 4.3 & 5.2 & 8.7 & 10.2 & 11.6 \\
%       Mem. (GB)    & 7.62 & 8.58 & 10.8 & 11.3 & 12.8 & 13.9 & 14.9 \\
%       SSIM (\%)    & 95.5 & 95.1 & 94.6 & 94.5 & 94.0 & 93.2 & 93.8  \\ 
      
%       \bottomrule
%     \end{tabular}
% }

{
  \centering
  \makeatletter
  % 1. 设置编号前缀为 A，并手动设定序号为 1
  \renewcommand{\thetable}{A\arabic{table}}
  \setcounter{table}{1}
  \def\@captype{table}
  \makeatother
  \footnotesize
  \setlength{\tabcolsep}{6pt}
  \renewcommand{\arraystretch}{0.9} % 稍微增加行间距，视觉更舒适
  
  % 2. 插入你要求的中文描述作为标题 (注意 & 符号需要加反斜杠 \&)
  \captionof{table}{\textbf{Variation across different numbers of input frames.}} 
\label{tab:number}
  \begin{tabular}{ccccccccc}
    \toprule
      Input Frames & 2 & 4 & 8 & 10 & 16 & 20 & 24 \\[-0.3ex]
      
      \midrule
      
      % === 数据 ===
      Time (s)    & 0.7 & 2.7 & 4.3 & 5.2 & 8.7 & 10.2 & 11.6 \\
      Mem. (GB)    & 7.62 & 8.58 & 10.8 & 11.3 & 12.8 & 13.9 & 14.9 \\
      SSIM (\%)    & 95.5 & 95.1 & 94.6 & 94.5 & 94.0 & 93.2 & 93.8  \\ 
    \bottomrule
  \end{tabular}
}
